Oracle-Efficient Smoothed Online Learning for Piecewise Continuous Decision Making

Smoothed online learning has emerged as a popular framework to mitigate the substantial loss in statistical and computational complexity that arises when one moves from classical to adversarial learning. Unfortunately, for some spaces, it has been shown that efficient algorithms suffer an exponentially worse regret than that which is minimax optimal, even when the learner has access to an optimization oracle over the space. To mitigate that exponential dependence, this work introduces a new notion of complexity, the generalized bracketing numbers, which marries constraints on the adversary to the size of the space, and shows that an instantiation of Follow-the-Perturbed-Leader can attain low regret with the number of calls to the optimization oracle scaling optimally with respect to average regret. We then instantiate our bounds in several problems of interest, including online prediction and planning of piecewise continuous functions, which has many applications in fields as diverse as econometrics and robotics.

==> body/body.tex <==
%!TEX root = ../main.tex

\section{Problem Setup \ac{OLD}}
We consider a general online learning setup with a fixed loss function $\ell: \Theta \times \cX \to \R$. At each time $t$, the learner selects a measure $\mu_t \in \Pclass$, and plays $\bx_t \sim \mu_t$. Simultaneously, the learner selects $\theta_t \in \Theta$. We define \emph{regret} as
\begin{align}
\reg_T := \sum_{t=1}^T \ell(\theta_t;\bx_t) - \inf_{\theta \in \Theta }\sum_{t=1}^T \ell(\theta;\bx_t). 
\end{align}
Let $\cI_{\tau} := \{(\tau-1)E,(\tau-1)E +1,\dots, \tau E -1\}$.
We define $\elltiltau := \sum_{t \in \cI_{\tau}}\ell_t$

\newcommand{\normc}[1]{\|#1\|_{\mathrm{c}}}
\newcommand{\normd}[1]{\|#1\|_{\mathrm{d}}}


\begin{definition} $\theta = (\thetac,\thetad)$. 
\end{definition}
\begin{assumption} For all $\bx \in \cX$ and $\thetac \in \Thetac$, $|\ell((\thetac,\thetad);\bx) -\ell((\thetac',\thetad);\bx)| \le \Lc \normc{\thetac - \thetac'}$
\end{assumption}
\begin{assumption}[Pseudo-Isometry]
\begin{align}
\sup_{\mu \in \Pclass}\Exp_{\bx \sim \mu}[|\ell((\thetac,\thetad) ; \bx) - \ell((\thetac,\thetad') ; \bx)| ] \le \alpha \normd{\thetad-\thetad'}^{\gamma} + \beta.
\end{align}
\end{assumption}
\begin{definition} $\Pclass$-$\cL_2$ covering of $\Thetac$. and Supremal cover in $\cL_1$ of $\Thetad$
\end{definition} 
\begin{assumption} Some bound on these covers.
\end{assumption}


\begin{condition}[Pseudo-Isometry]
\begin{align}
\ee\left[ \elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1}) \right] \leq \alpha \cdot \ee\left[ \normd{\theta_\tau - \theta_{\tau+1}}^{\gamma} \right] + \gamma.
\end{align}
\end{condition}





\subsection{Stuff}
We assume that $\theta = (\thetac,\thetad) \in \Thetac \times \Thetad$ decomposes into a ``discrete'' and a ``continuous'' component, such that $\theta \mapsto \ell(\theta;\bx)$ is Lipschitz in $\thetac$.


$\ell_t(g_{\phi}(\theta;\bx);\bx)$. 

We consider two classes of problems.
\paragraph{Piecewise Smooth Functions}

$\cG := \bigcup_{k}\cG_k, \quad \cG_k: \{\}$
We consider a function of the form
\begin{align}
\gphi(\theta;\bx) := g(\theta,\kphi(\theta;\bx);\bx), \quad \kphi(\theta;\bx) = \argmax_{k \in [K]} \varphi(\theta,k;\bx),
\end{align}
and loss functions 
\begin{align}
\ell_{t}(\bx;\theta) = c_t(\gphi(\theta;\bx)).
\end{align}
and $\ell:\R^d \to \R$ is a smooth loss. An example is piecewise affine regresion. Here, we let $\theta = (\bV, \bW)$, with 
\begin{align}
\varphi(\bW,k;\bx) &=  \langle \bW[k], \bx \rangle , \quad 
g(\bV;\bx) = \bV \bx, \quad c_t(\bz) = \|\bz\|^2.
\end{align}


\paragraph{Piecewise Smooth Planning}
\begin{align}
\bz_t^{(h+1)} = f^{(h)}(\theta;\bw^{(h)},\bz_t^{(h)}),  \quad f^{(h)} = g^{(h)}_{\phi^{(h)}}, \quad \bx_t = (\bw_t^{(1:h)},\bz_t^{(0)})
\end{align}
and 
\begin{align}
\ell_t(\bx_t;\theta) = c_{t}(\bz_{t}^{(1:h)})
\end{align}
\section{Main Result}
Let $\Pclass$ be a family of distributions over $\cX$. We say that a sequence of random variables $(\bx_{\blockstep})_{\blockstep \ge 1}$ are $\Pclass$-adapted if there exists a filtration $(\cF_{\blockstep})_{\blockstep \ge 1}$ such that $\bx_{\blockstep}$ is $\cF_{\blockstep}$-adapted and if the distribution of $\bx_{\blockstep} \mid \cF_{\blockstep-1}$ lies in $\Pclass$. Let $\dist(\cdot,\cdot ; \bx): \Theta \times \Theta \to \R_{\ge 0}$ be a family of pseudometrics parameterized by $\bx \in \cX$. We define the pseudometric
\begin{align}
\distpp[p](\cdot,\cdot) := \sup_{\mu \in \Pclass}\Exp_{\bx \sim \mu}[\dist(\cdot,\cdot;\bx)^p]^{1/p}
\end{align}

\newcommand{\cover}{\scrN}
\newcommand{\thetset}{\scrT}
\begin{definition} We say that a finite set $\cover = (\theta_i,\thetset_i)_{i=1}^N \subset \Theta \times 2^{\Theta} $ is an $\epsilon$-supremal cover under $\Pclass$ if $\bigcup_{i=1}^M \Theta_i = \Theta$ and 
\begin{align}
\forall i \in [N], \quad \sup_{\mu \in \Pclass}\Exp_{\bx \sim \mu}\Exp\left[\sup_{\theta \in \thetset_i}\dist(\theta,\theta_i;\bx)\right] \le \epsilon
\end{align}
\end{definition}
\begin{assumption}\label{asm:R_bound} We assume $\dist(\cdot,\cdot;\bx) \le R$.
\end{assumption}

\begin{proposition}\label{prop:dis_cov}
Let $N(\epsilon)$ denote the minimal cardinality of an $\epsilon$-supremal cover of cardinality over $\Theta$ under $\Pclass$. Then, with probability $1-\delta$, the following holds for all $\theta,\theta' \in \Theta$ simultaneously:
\begin{align}
\left|\frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta,\theta';\bx_{\blockstep})\right| &\le 2\distpp[1](\theta,\theta') + \inf_{\epsilon > 0}\left( 8\epsilon  + \frac{3R\log(4N(\epsilon)^2/\delta)}{ \block}\right)
\end{align}
\end{proposition}

\begin{assumption} $\distpp(\theta,\theta') \le \kappa \|\theta - \theta'\|$
\end{assumption}
\subsection{Proof of Proposition \ref{prop:dis_cov} }
 \url{http://www.satyenkale.com/papers/minimonster.pdf}
We begin with Freedman's Inequality,
\begin{lemma}[Freedmans Inequality] Let $Z_1,\dots,Z_n$ be martingale sequence such $|Z_{\blockstep}| \le R$ almost surely, and $\Exp[Z_{\blockstep}^2 \mid Z_{1:h-1}] \le \sigma^2$. 
\begin{align}
\frac{1}{\block}\sum_{\blockstep=1}^{\block} Z_{\blockstep} \le \left(\frac{\sigma^2}{ R} + \frac{ R\log(1/\delta)}{B} \right)
\end{align}
\end{lemma}
\begin{proof}[Proof of Proposition \ref{prop:dis_cov}] Throughout, we use that
\begin{align}
\distpp[2](\theta,\theta')^2 \le R\distpp[1](\theta,\theta'),
\end{align}
which follows from \Cref{asm:R_bound}. Define the random processes
\begin{align}
Y_{\blockstep}(\theta,\theta') &:= \dist(\theta,\theta';\bx_{\blockstep})\\
Z_{\blockstep}(\theta,\theta') &:= Y_{\blockstep}(\theta,\theta') - \Exp_{\bx_{\blockstep}}[Y_{\blockstep}(\theta,\theta') \mid \cF_{\blockstep-1}]
\end{align}


\Cref{asm:R_bound} implies that  $|Z_{\blockstep}(\theta,\theta';\bx)| \le R$ almost surely. Moreover, as $\bx_{1:n}$ is $\Pclass$-adapted, we have $\Exp[Z_{\blockstep}(\theta,\theta';\bx)^2 \mid \cF_{\blockstep-1}] \le \distpp[2](\theta,\theta')^2 \le R\distpp[1](\theta,\theta')$. Thus, Freedman's inequality gives
\begin{align}
\Pr\left[\frac{1}{\block}\sum_{\blockstep=1}^{\block} Z_{\blockstep}(\theta,\theta';\bx_{\blockstep}) \le  \left(\distpp[1](\theta,\theta') + \frac{R\log(1/\delta)}{\block} \right)\right] \ge 1 - \delta.
\end{align}
Moreover, as $Z_{\blockstep}(\theta,\theta') \le Y_{\blockstep}(\theta,\theta') + \Exp_{\bx_{\blockstep}}[Y_{\blockstep}(\theta,\theta') \mid \cF_{\blockstep-1}] \le Y_{\blockstep}(\theta,\theta') + \distpp[1](\theta,\theta')$, by a union bound, the following event holds with probability at least $1 - \delta/2$:
\begin{align}
\cE_1 := \left\{\forall i, j \in [N], \quad  \frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta_i,\theta_j;\bx_{\blockstep})\le 2\distpp[1](\theta_j,\theta_j) + \frac{R\log(4N^2/\delta)}{\alpha n} \right\} 
\end{align}
Next, define the processes 
\begin{align}
Y_{\blockstep,i}(\bx_{\blockstep}) := \sup_{\theta \in \thetset_i} \dist(\theta,\theta_i; \bx_{\blockstep}) \quad  Z_{\blockstep,i} := Z_{\blockstep,i}(\bx_{\blockstep}) - \Exp[Z_{\blockstep,i}(\bx_{\blockstep}) \mid \cF_{\blockstep-1}].
\end{align} Observe that $Z_{\blockstep,i} \in [-R,R]$. Moreover, $\Exp[Z_{\blockstep,i}^2 \mid \cF_{\blockstep-1}] \le \Exp[Y_{\blockstep,i}^2 \mid \cF_{\blockstep-1}] \le R \Exp[Y_{\blockstep,i} \mid \cF_{\blockstep-1}] \le R\epsilon$ by definition of the cover. Hence, Friedman's inequality gives
\begin{align}
\Pr\left[\frac{1}{\block}\sum_{\blockstep=1}^{\block}  Z_{\blockstep,i}\le  \epsilon + \frac{R\log(1/\delta)}{\block} \right] \ge 1 - \delta.
\end{align}
so that, using $\Exp[Y_{\blockstep,i} \mid \cF_{\blockstep-1}] \le \epsilon$ by the definition of the cover and substituting $Y_{\blockstep,i}= \sup_{\theta \in \thetset_i} \dist(\theta,\theta_i; \bx_{\blockstep})$, 
\begin{align}
\Pr\left[\frac{1}{\block}\sum_{\blockstep=1}^{\block}  \sup_{\theta \in \thetset_i} \dist(\theta,\theta_i; \bx_{\blockstep})\le 2\epsilon + \frac{R\log(1/\delta)}{\block}\right] \ge 1 - \delta.
\end{align}
Thus, a union bound over $i \in [N]$, and moving the supremum outside the sum implies that the following event holds with probability at least $1 - \delta/2$:
\begin{align}
\cE_2 := \left\{\max_{i \in [M]}\frac{1}{\block}\sup_{\theta \in \thetset_i} \sum_{\blockstep=1}^{\block}  \dist(\theta,\theta_i; \bx_{\blockstep})\le 2\epsilon + \frac{R\log(2N/\delta)}{ n} \right\} 
\end{align}
On $\cE_{1} \cap \cE_2$, we then have that for any $\theta, \theta'$ with $\theta \in \thetset_i$ and $\theta' \in \thetset_j$ that
\begin{align}
\frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta,\theta';\bx_{\blockstep}) &\le  \frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta,\theta_i;\bx_{\blockstep}) + \dist(\theta',\theta_j;\bx_{\blockstep}) + \dist(\theta',\theta_j';\bx_{\blockstep})\\
&\le  4\epsilon + 2\distpp[1](\theta_i,\theta_j) + \frac{3R\log(4N^2/\delta)}{ n} 
\end{align}
To conclude, we apply the triangle inequality again to bound that $\distpp[1](\theta_i,\theta_j) \le \distpp[1](\theta_i,\theta) + \distpp[1](\theta_j,\theta') + \distpp[1](\theta,\theta') \le 2\epsilon + \distpp[1](\theta,\theta')$.  Hence, on $\cE_1 \cap \cE_2$,
\begin{align}
\frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta,\theta';\bx_{\blockstep}) &\le  \frac{1}{\block}\sum_{\blockstep=1}^{\block} \dist(\theta,\theta_i;\bx_{\blockstep}) + \dist(\theta',\theta_j;\bx_{\blockstep}) + \dist(\theta',\theta_j';\bx_{\blockstep})\\
&\le  8\epsilon + 2\distpp[1](\theta,\theta') + \frac{3R\log(4N^2/\delta)}{ n}. 
\end{align}
\end{proof}



\section{Be The Leader}
In this section, we show that if the adversary is oblivious, then a lazy FTPL algorithm can still achieve competitive regret using the Be-The-Leader lemma \citep{kalai2005efficient}.  Suppose that we are in the online learning setting where at each time $1 \leq t \leq T$, the adversary chooses $x_t \in \cX$ and the learner chooses $\theta_t \in \Theta$.  Given a fixed and known loss function $\ell: \Theta \times \cX \to \rr$, the goal of the learner is to minimize expected regret:
\begin{align}
    \reg_T = \sum_{t = 1}^T \ell(\theta_t, x_t) - \inf_{\theta \in \Theta} \sum_{t=  1}^T \ell(\theta, x_t).
\end{align}
We abbreviate $\sum_{s = 1}^t \ell(\theta, x_s) = L_t(\theta)$.  Suppose that there are some possibly random perturbations $\omega_t: \Theta \to \rr$.  Then the following lemma from \citet{block2022smoothed}, which generalizes the Be-the-Leader lemmas from \citet{kalai2005efficient,cesa2006prediction}, holds:
% \begin{lemma}[Be-The-Leader Lemma]\label{lem:btl}
%     Let $n \in \bbN$ and suppose for each $1 \leq \tau \leq T / n$, the learner chooses some approximate minimizer of the perturbed cumulative loss.  More precisely, for some real-valued function $\gamma$ on the stochastic process, the learner chooses some $\theta_\tau$ satisfying
%     \begin{align}\label{eq:ftpl}
%         L_{(\tau - 1) \cdot n}(\theta_\tau) + \omega_{(\tau - 1) \cdot n + 1 }(\theta_\tau) \leq \gamma(\omega_{\tau - 1} \cdot n + 1) + \inf_{\theta \in \Theta} L_{(\tau - 1) \cdot n}(\theta) + \omega_{(\tau - 1) \cdot n + 1 }(\theta)
%         % \theta_\tau \in \argmin_{\theta \in \Theta} L_{(\tau - 1) \cdot n}(\theta) + \omega_{(\tau - 1) \cdot n + 1 }(\theta)
%     \end{align}
%     and plays $\theta_\tau$ for all $(\tau - 1) \cdot n + 1 \leq t \leq \tau  \cdot n$.  Suppose that the $\omega_t$ are independent and identically distributed random processes on $\Theta$ satisfying $\ee\left[ \sup_{\theta \in \Theta} \omega_t(\theta) \right] \geq 0$.  Then, the learner experiences the following regret:
%     \begin{align}
%         \ee\left[ \reg_T \right] \leq  \frac{T}{n} \cdot \ee\left[ \gamma(\omega_1) \right] +  \ee\left[ \sup_{\theta} \omega_1(\theta) \right] + \sum_{\tau = 1}^{T / n} \ee\left[ \sum_{t = (\tau - 1) \cdot n + 1}^{\tau \cdot n} \ell(\theta_\tau, x_t) - \ell(\theta_{\tau+1}, x_t) \right]
%     \end{align}
% \end{lemma}
% \begin{proof}
%     We apply the proof of \citet[Lemma 31]{block2022smoothed} to the cumulative loss over $n$ steps.  Thus, for each $1 \leq \tau \leq T' = \floor{T / n}$, let
%     \begin{align}
%         \elltil_\tau(\theta) = \sum_{t = (\tau - 1) \cdot n + 1}^{\tau \cdot n} \ell(\theta, x_t).
%     \end{align}
%     We will apply induction on $T'$ to the inequality
%     \begin{align}\label{eq:inductionbtl}
%         \ee\left[ \sum_{\tau = 1}^{T'} \elltil_\tau(\theta_{\tau + 1}) \right] \leq \ee\left[ \sum_{\tau = 1}^{T'} \ell_\tau(\theta_{T' + 1}) + \omega_{T'\cdot n + 1}(\theta_{T' + 1}) \right] + \ee\left[ \sup_{\theta \in \Theta} \omega_{1}(\theta) \right] + \frac{T'}{n} \cdot \ee\left[ \gamma(\omega_1) \right].
%     \end{align}
%     For the base case of $T' = 0$ the statement is trivial.  Suppose that for some fixed $T' -1$ that \eqref{eq:inductionbtl} holds.  Then we see by construction that
%     \begin{align}
%         \ee\left[ \sum_{\tau = 1}^{T' - 1} \elltil_\tau(\theta_{T'}) + \omega_{T'\cdot n + 1}(\theta_{T'}) \right] &\leq \ee\left[ \inf_{\theta \in \Theta} \sum_{\tau = 1}^{T' - 1} \elltil_\tau(\theta) + \omega_{T'}(\theta) \right] + \ee\left[ \gamma)\omega_{T'} \right]\\
%         &\leq \ee\left[ \sum_{\tau = 1}^{T' - 1} \elltil\left( \theta_{T' + 1} \right) + \omega_{(T' + 1) \cdot n + 1}\left( \theta_{T' + 1} \right) \right] + \ee\left[ \gamma(\omega_{(T' + 1) \cdot n + 1}) \right],
%     \end{align}
%     where the second inequality follows from the fact that the $\omega_t$ are independent and identically distributed as well as the construction of $\theta_{T' + 1}$.  Combining the induction hypothesis \eqref{eq:inductionbtl} with the above inequality tells us that
%     \begin{align}
%         \ee\left[ \sum_{\tau = 1}^{T' - 1} \elltil_\tau(\theta_{\tau + 1}) \right] \leq \ee\left[ \sum_{\tau = 1}^{T' - 1} \elltil_\tau\left( \theta_{T' + 1} \right) + \omega_{(T' + 1) \cdot n + 1}\left( \theta_{T' + 1} \right) \right] + \ee\left[ \sup_{\theta \in \Theta} \omega_1(\theta) \right] + \frac{T'}{n} \cdot \ee\left[ \gamma(\omega_1) \right].
%     \end{align}
%     Adding $\ee\left[ \elltil_{T'}(\theta_{T' + 1}) \right]$ to both sides finishes the induction proof.

%     To continue, we compute:
%     \begin{align}
%         \ee\left[ \sum_{\tau = 1}^{T'} \elltil_\tau(\theta_{T' + 1}) + \omega_{T'  + 1}(\theta_{T' + 1}) \right] &\leq \ee\left[ \inf_{\theta \in \Theta} \sum_{\tau = 1}^{T'} \elltil_\tau\left( \theta \right) + \sup_{\theta' \in \Theta} \omega_1(\theta) \right] +\frac{T'}{n} \cdot \ee\left[ \gamma(\omega_1) \right]\\
%         &\leq \ee\left[ \inf_{\theta \in \Theta} \sum_{t = 1}^T \ell(\theta, x_t) \right] + \ee\left[ \sup_{\theta \in \Theta} \omega_1(\theta) \right]\frac{T'}{n} \cdot \ee\left[ \gamma(\omega_1) \right],
%     \end{align}
%     where we used the construction of $\theta_{T' + 1}$ for the first inequality and the definition of $\elltil_\tau$ for the second inequality.  To conclude, we apply \eqref{eq:inductionbtl} and observe:
%     \begin{align}
%         \ee\left[ \reg_T \right] &= \ee\left[ \sum_{t = 1}^T \ell(\theta_{\tau(t)}) - \inf_{\theta \in \Theta} \sum_{t = 1}^T \ell(\theta, x_t) \right] \\
%         &\leq \ee\left[ \sum_{\tau = 1}^{T'} \elltil_\tau(\theta_\tau) \right] - \ee\left[ \sum_{\tau = 1}^{T'} \elltil_\tau(\theta_{\tau + 1}) \right] + 2 \ee\left[ \sup_{\theta \in \Theta} \omega_1(\theta) \right] + \frac{T'}{n} \cdot \ee\left[ \gamma(\omega_1) \right],
%     \end{align}
%     where we denoted by $\tau(t) = \floor{t / n}$.  The result follows from the construction of $\elltil_\tau$.
% \end{proof}


\section{Follow The Perturbed Leader}
In this section we apply the proof technique of \citet{suggala2020online} to losses that are not necessarily Lipschitz.    In particular, we let $\xi_t \sim \expo(1)$ denote a random vector in $\rr^d$ with coordinates sampled independently according to an exponential distribution.  We let $\omega_t(\theta) = -\eta \inprod{\xi}{\theta}$ for some $\eta > 0$.  We instantiate \eqref{eq:ftpl}, where for some fixed $n$, for each $1 \leq \tau \leq T'$, we let $\theta_\tau(\xi)$ be some approximate minimizer of the perturbed cumulative loss.  More precisely, for some real-valued function on $\rr^d$, we suppose that
% \begin{align}\label{eq:thetaxi}
%     L_{(\tau - 1) \cdot n}(\theta_\tau(\xi)) - \eta \inprod{\xi}{\theta_\tau(\xi)} \leq \gamma(\xi) +  \inf_{\theta \in \Theta} L_{(\tau - 1) \cdot n}(\theta) - \eta \inprod{\xi}{\theta}
%     % \theta_\tau(\xi) \in \argmin_{\theta \in \Theta} L_{(\tau - 1) \cdot n}(\theta) - \eta \inprod{\xi}{\theta}
% \end{align}
% and we predict by sampling $\xi \sim \expo(1)$ and predicting $\theta_\tau = \theta_\tau(\xi)$.  Note that $\elltil_\tau(\theta)$ is not necessarily Lipschitz and so we cannot directly apply the results of \citet{suggala2020online}.  We can, however, modify their technique:
% \begin{lemma}%\label{lem:monotonicity1}
%     Suppose that $\xi, \xi' \in \rr^d$ with $\theta = \theta_\tau(\xi)$ and $\theta' = \theta_\tau(\xi')$ for some fixed $\tau$, as in \eqref{eq:thetaxi}.  Then the following inequality holds:
%     \begin{align}
%         \eta \cdot\inprod{\xi' - \xi}{\theta' - \theta} \geq - \left( \gamma(\xi) + \gamma(\xi') \right).
%     \end{align}
% \end{lemma}
% \begin{proof}
%     We abbreviate
%     \begin{align}
%         \Ltil_\tau(\theta) = \sum_{\tau' = 1}^\tau \elltil_{\tau'}(\theta)
%     \end{align}
%     and compute:
%     \begin{align}
%         \Ltil_\tau(\theta) - \eta \inprod{\xi}{\theta} &\leq \Ltil_\tau(\theta') - \eta \inprod{\xi}{\theta'} + \gamma(\xi) \\
%         &= \Ltil_\tau(\theta') - \eta \inprod{\xi'}{\theta'} + \eta \inprod{\xi' - \xi}{\theta'} + \gamma(\xi) \\
%         &\leq \Ltil_\tau(\theta) - \eta \inprod{\xi'}{\theta} + \eta \inprod{\xi' - \xi}{\theta'}+ \gamma(\xi) + \gamma(\xi').
%     \end{align}
%     The result follows.
% \end{proof}
% The second monotonicity lemma corresponds to \citet[Lemma 6]{suggala2020online} and is proved similarly:
% \begin{lemma}\label{lem:monotonicity2}
%     Suppose that $\xi,\xi' \in \rr^d$ with $\theta_\tau = \theta_\tau(\xi)$, $\theta_{\tau'} = \theta_\tau(\xi')$ and $\theta_{\tau+1}, \theta_{\tau+1}'$ defined similarly for some fixed $\tau$.  Then the following inequality holds:
%     \begin{align}
%         \min\left( \inprod{\theta_\tau'}{\xi' - \xi}, \inprod{\theta_{\tau+1}'}{\xi' - \xi} \right) \geq \max\left( \inprod{\theta_\tau}{\xi' - \xi}, \inprod{\theta_{\tau+1}}{\xi' - \xi} \right) - \frac{2\left( \gamma(\xi) + \gamma(\xi') \right) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau + 1})}}\eta.
%     \end{align}
% \end{lemma}
% \begin{proof}
%     By construction, we compute:
%     \begin{align}
%         \Ltil_{\tau}(\theta_\tau) - \eta \inprod{\xi}{\theta_\tau} &= \Ltil_{\tau - 1}(\theta_\tau) - \eta \inprod{\xi}{\theta_\tau} + \elltil_\tau(\theta_\tau) \\
%         &\leq \Ltil_{\tau - 1}(\theta_{\tau + 1}) - \eta \inprod{\xi}{\theta_{\tau + 1}} + \elltil_\tau(\theta_\tau) + \gamma(\xi) \\
%         &= \Ltil_\tau(\theta_{\tau + 1}) - \eta \inprod{\xi}{\theta_{\tau + 1}} + \gamma(\xi) + \elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau + 1}).
%     \end{align}
%     Again by construction, we have:
%     \begin{align}
%         \Ltil_\tau(\theta_\tau) - \eta \inprod{\xi}{\theta_\tau} &= \Ltil_\tau(\theta_\tau) - \eta \inprod{\xi'}{\theta_\tau} + \eta \inprod{\xi' - \xi}{\theta_\tau} \\
%         &\geq \Ltil_\tau(\theta_{\tau+1}') - \eta \inprod{\xi'}{\theta_{\tau + 1}'} + \eta \inprod{\xi' - \xi}{\theta_\tau} - \gamma(\xi') \\
%         &= \Ltil_\tau(\theta_{\tau +1}') - \eta \inprod{\xi}{\theta_{\tau + 1}'}  + \eta \inprod{\xi' - \xi}{\theta_\tau - \theta_{\tau +1}'} - \gamma(\xi') \\
%         &\geq \Ltil_\tau(\theta_{\tau + 1}) - \eta \inprod{\xi}{\theta_{\tau + 1}}+ \eta \inprod{\xi' - \xi}{\theta_\tau - \theta_{\tau +1}'} - \gamma(\xi').
%     \end{align}
%     Combining the two preceding displays leads to the following inequality:
%     \begin{align}
%         \eta\inprod{\xi' - \xi}{\theta_\tau - \theta_{\tau + 1}'} \geq - 2\left( \gamma(\xi) + \gamma(\xi') \right) - \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau +1})}.
%     \end{align}
%     An identical argument yields
%     \begin{align}
%         \eta\inprod{\xi' - \xi}{\theta_\tau' - \theta_{\tau + 1}} \geq - 2\left( \gamma(\xi) + \gamma(\xi') \right) - \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau +1})}.
%     \end{align}
%     Applying Lemma \ref{lem:monotonicity1} gives
%     \begin{align}
%         \eta\inprod{\xi' - \xi}{\theta_\tau' - \theta_\tau} &\geq - \left( \gamma(\xi) + \gamma(\xi') \right) \\
%         \eta\inprod{\xi' - \xi}{\theta_{\tau + 1}' - \theta_{\tau + 1}} &\geq - \left( \gamma(\xi) + \gamma(\xi') \right).
%     \end{align}
%     Combining the inequalities concludes the proof.
% \end{proof}
% Using the two monotonicity results above, we have the following lemma:
% \begin{lemma}%\label{lem:stability1}
%     Suppose that $\theta_\tau \in \rr^d$ is chosen according to \eqref{eq:thetaxi}.  Suppose further that the $\ell^\infty$ diameter of $\Theta$ is bounded above by $D$.  Then it holds for any $k > 0$,
%     \begin{align}
%         \ee\left[ \norm{\theta_\tau - \theta_{\tau + 1}}_1 \right] \leq  k d D + d \cdot \ee\left[\frac{2(\gamma(\xi) + \gamma(\xi')) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau + 1})} }{\eta k}\right].
%     \end{align}
% \end{lemma}
% \begin{proof}
    % For some fixed $\tau$ and $\xi$, for all $1 \leq i \leq d$, let
    % \begin{align}
    %     \thetamax = \max(\theta_{\tau,i}, \theta_{\tau+1,i}), && \thetamin = \min(\theta_{\tau,i}, \theta_{\tau+1,i})
    % \end{align}
    % and observe that $\abs{\theta_{\tau,i} - \theta_{\tau+1,i}} = \thetamax - \thetamin$.  Suppose that $\xi \sim \expo(1)$ and let $\xi' = \xi + k \be_i$.  Then, using the memoryless property of the exponential distribution and denoting
    % \begin{align}
    %     \ee_{-i}[\cdot] = \ee\left[ \cdot | \xi_1, \dots, \xi_{i-1}, \xi_{i+1}, \dots, \xi_d \right],
    % \end{align}
    % we have
    % \begin{align}
    %     \ee_{-i}\left[ \thetamin \right] &= \pp\left( \xi_i \leq k \right) \cdot \ee_{-i}\left[ \thetamin | \xi_i \leq k \right] + \pp\left( \xi_i >k \right) \cdot \ee_{-i}\left[ \thetamin | \xi_i > k \right] \\
    %     &\geq \left( 1 - e^{-k} \right) \left( \ee_{-i}\left[ \thetamax \right] - D\right) + e^{-k} \cdot \ee_{-i}\left[ \thetamin | \xi_i > k \right]\\
    %     &= \left( 1 - e^{-k} \right) \left( \ee_{-i}\left[ \thetamax \right] - D\right) + e^{-k} \cdot\ee\left[ \thetamin' \right]
    % \end{align}
    % where $\thetamin' = \thetamin(\xi')$.  The inequality follows from the assumption on the diameter of $\Theta$ and the second equality follows from the memoryless property of the exponential distribution.  Applying Lemma \ref{lem:monotonicity2} and observing that $\inprod{\theta_\tau}{\xi' - \xi} = k \theta_{\tau,i}$, we see that
    % \begin{align}
    %     \ee_{-i}\left[ \thetamin' \right] &\geq \ee_{-i}\left[ \thetamax \right] - \ee_{-i}\left[\frac{2 (\gamma(\xi) + \gamma(\xi')) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1})}}{\eta k}\right].
    % \end{align}
    % Thus, combining the previous displays tells us that
    % \begin{align}
    %     \ee_{-i}\left[ \thetamin \right] \geq \ee_{-i}[\thetamax] - \left( 1 - e^{-k} \right)D - \ee_{-i}\left[\frac{2 (\gamma(\xi) + \gamma(\xi')) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1})}}{\eta k}\right].
    % \end{align}
    % Then,
    % \begin{align}
    %     \ee_{-i}\left[ \abs{\theta_{\tau,i} - \theta_{\tau+1,i}} \right] &= \ee_{-i}\left[ \thetamax - \thetamin \right] \\
    %     &\leq \left( 1 - e^{-k} \right)D + \ee_{-i}\left[\frac{2 (\gamma(\xi) + \gamma(\xi')) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1})}}{\eta k}\right] \\
    %     &\leq k D + \ee_{-i}\left[\frac{2 (\gamma(\xi) + \gamma(\xi')) + \abs{\elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1})}}{\eta k}\right].
    % \end{align}
    % Summing over $1 \leq i \leq d$ concludes the proof.
% \end{proof}
We can now prove the nonconvex, non-Lipschitz FTPL bound:
\begin{theorem}\label{thm:ftpl}
    Suppose that for all $\tau$ that $\elltil_\tau$ satisfies the following bound for some nonnegative constants $(\alpha, \beta)$:
    \begin{align}
        \ee\left[ \elltil_\tau(\theta_\tau) - \elltil_\tau(\theta_{\tau+1}) \right] \leq \alpha \cdot \ee\left[ \norm{\theta_\tau - \theta_{\tau+1}}_1 \right] + \beta.
    \end{align}
    Then if the learner plays $\theta_\tau$ in epoch $\tau$ of length $n$, the expected regret is bounded as follows:
    \begin{align}
        \ee\left[ \reg_T \right] \leq \frac{T}{n} \cdot \left( \ee\left[ \gamma(\eta \xi) \right] + \frac{\beta}{2 \alpha} + \frac{\gamma(\eta\xi) + \gamma(\eta\xi')}{\alpha} \right) + \eta \cdot \ee\left[ \sup_{\theta \in \Theta} \inprod{\xi}{\theta} \right] + \frac{2 \alpha d^2 D T}{\eta n}.
    \end{align}
\end{theorem}
\begin{proof}
    Set $k = 2 \alpha d$ in Lemma \ref{lem:stability1} and aLemma \ref{lem:{lem:btl}.
\end{proof}

==> body/old.tex <==


\subsection{New}
\newpage
Let $\ell(\theta;\bx_i,\bw)$ satisfy $\Exp_{\bw \sim \mu}\ell(\theta;\bx,\bw) = 0$. 
Consider functions of the form
\begin{align*}
L(\theta;\bx_{1:n},\bw_{1:n}) &= \sum_{h=1}^n \ell(\theta;\bx_h,\bw_h) , \quad 
\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n}) := L(\theta;\bx_{1:n},\bw_{1:n}) - L(\theta';\bx_{1:n},\bw_{1:n}).
\end{align*}
Introduce
\begin{align*}
\dtwo(\theta,\theta';\bx_{1:n}) := \sqrt{\frac{1}{n}\sum_{h=1}^n\Exp_{\bw \sim \mu}\left[\left(\ell(\theta;\bx_h,\bw) -\ell(\theta';\bx_h,\bw)\right)^2\right]}
\end{align*}

\begin{definition}[Disagreement Cover]Fix $\bx_{1:n}$. We say that $\cT := \{(\theta_i,\cD_{i,1:n})\}_{i \in [|\cT|]} \subset \Theta \times \cW^n$ is an $\beps =(\epsmu,\epsl)$-disagreement cover of $\Theta$ in the norm $\|\cdot\|$, if 
\begin{itemize}
	\item[(a)]  $\max_{i}\frac{1}{n}\sum_{h=1}^n \Pr_{\mu}[\bw \in \cD_{i,h}] \le \epsmu$.
\end{itemize}
and for every $\theta \in \Theta$, there exists an $i = i_{\cT}(\theta) \in [|\cT|]$ such that, 
\begin{itemize}
	\item[(b)] $\frac{1}{n}\sum_{h=1}^n\sup_{\bw \in \cD_{i,h}}|\ell(\theta;\bx_j,\bw) - \ell(\theta_i;\bx_h,\bw)|^2 \le \epsl^2$.
	%\item[(c)] $\|\theta_i - \theta\| \le \epsnrm$
\end{itemize}
\end{definition} 
\begin{assumption} $\sup_{\bx,\bw,\theta}|\ell(\theta;\bx,\bw)| \le B$. 
\end{assumption}

\begin{proposition}\label{prop:uniform_dev} Let $\cT$ be a $(\epsmu,\epsl)$-disagreement cover of cardinality $M$, with $\epsl \le B$. Then, with probability at least $1 - 2\delta$, the following holds for all $\theta,\theta' \in \Theta$
\begin{align*}
|\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n}))| \le \inf_{\alpha > 0 } 4(1+\alpha^{-1})(\epsl + B\epsmu) + \frac{\dtwo(\theta,\theta';\bx_{1:n})^2}{2\alpha B} +   \frac{(4+3\alpha)B\log(2M/\delta)}{3n}
\end{align*}
\end{proposition}

\subsection{Proof of Proposition \ref{prop:uniform_dev}}

\begin{lemma} Let $\cT \subset \Theta$ be a finite set. Then, with probability $1-\delta$, it holds that 
\begin{align*}
\Pr_{\bw_{1:n} \sim \mu}\left[\forall \theta,\theta' \in \Theta,  ~|\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n})| \le \dtwo(\theta,\theta';\bx_{1:n})\sqrt{2\frac{\log(2|\cT|/\delta)}{n}} + \frac{B\log(2|\cT|/\delta)}{3n}\right] \ge 1- \delta.
\end{align*}
\end{lemma}

\mscomment{can actually remove obliviousness}
\begin{lemma} Let $\cT$ be a $\beps$-disagreement cover of $\Theta$ for $\bx_{1:n}$ fixed, and let $|\ell(\cdot)| \le B$ and $M = |\cT|$. Then, 
\begin{align*}
\Pr_{\bw_{1:n} \sim \mu}\left[\sup_{\theta} |\Delta(\theta,\theta_{i_{\cT}(\theta)};\bx_{1:n},\bw_{1:n}))| \ge \epsl +  2B\epsmu + \frac{B\log(M/\delta)}{2n} \right] \le \delta.
\end{align*}
\end{lemma}
\begin{proof} Let $\Theta_i := \{\theta \in \Theta: i_{\cT}(\theta) = i\}$, $M = |\cT|$ and define the increments
\begin{align*}
Z_{i,h} := \sup_{\theta \in \Theta_i}|\ell(\theta;\bx_h,\bw_h) - \ell(\theta_i;\bx_h,\bw_h)|
\end{align*}
Then, it holds that
\begin{align*}
\sup_{\theta} |\Delta(\theta,\theta_{i_{\cT}(\theta)};\bx_{1:n},\bw_{1:n}))| \le \max_{i \in [M]} \frac{1}{n}\sum_{h=1}^n Z_{i,h}. 
\end{align*}
Define the event $\cE_{i,h} := \I\{\bw_{h} \notin \cD_{i,h}\}$. Then, by the definition of a disagreement cover and Jensen's inequality,
\begin{align*}
\frac{1}{n}\sum_{h=1}^n Z_{i,h} &= \frac{1}{n}\sum_{h=1}^nZ_{i,h}\I\{\cE_{i,h}\} + \frac{1}{n}\sum_{h=1}^nZ_{i,h}\I\{\cE_{i,h}\}\\
&= \sqrt{\frac{1}{n}\sum_{h=1}^nZ_{i,h}^2\I\{\cE_{i,h}^c\}} + \frac{B}{n}\sum_{h=1}^n\I\{\cE_{i,h}\}\\
&= \epsl + \frac{B}{n}\sum_{h=1}^n\I\{\cE_{i,h}\},
\end{align*}
so that
\begin{align*}
\sup_{\theta} |\Delta(\theta,\theta_{i_{\cT}(\theta)};\bx_{1:n},\bw_{1:n}))| \le \epsl + \frac{B}{n}\sum_{h=1}^n\I\{\cE_{i,h}\} \numberthis\label{eq:Del_cover}
\end{align*}
	By definition of the disagreement, $\frac{1}{n}\sum_{h=1}^n\Pr[\cE_{i,h}] \le \epsmu$. Thus, Lemma D.2 in \mscomment{chernoff thing} implies that fixed $i$, we have that, with probability at least $1 - \delta$, for any fixed $i$,
\begin{align*}
\Pr_{\bw_{1:n} \sim \mu}\left[\frac{1}{n}\sum_{h=1}^n\I\{\cE_{i,h}\} \ge  2\epsmu + \frac{\log(1/\delta)}{2n} \right] \le \delta.
\end{align*}
Hence, by a union bound and \Cref{eq:Del_cover}, 
\begin{align*}
\Pr_{\bw_{1:n} \sim \mu}\left[\sup_{\theta}| \Delta(\theta,\theta_{i_{\cT}(\theta)};\bx_{1:n},\bw_{1:n}))| \ge \epsl +  2B\epsmu + \frac{B\log(M/\delta)}{2n} \right] \le \delta.
\end{align*}
\end{proof}
\begin{lemma} Let $\cT$ be an  $\beps =(\epsmu,\epsl)$-disagremment cover of $\Theta$ given $\bx_{1:n}$. Then, 
\begin{align*}
\dtwo(\theta,\theta_{i_{\cT}(\theta)};\bx_{h})^2 \le \epsl^2 + B^2\epsmu
\end{align*}
\end{lemma}
\begin{proof} Fix $\theta$, and let $\theta_i = \theta_{i_{\cT}(\theta)}$. Define $Z_h(bw) := \ell(\theta;\bx_h,\bw) - \ell(\theta_i;\bx_h,\bw)$. Then, $\dtwo(\theta,\theta_i;\bx_{h})^2 \le \max_{h \in [n]}\Exp[Z_{h}(\bw)^2] $. Using the definition of a disagreement cover, we bound $\frac{1}{n}\sum_{h=1}^n\Exp[Z_{h}(\bw)^2] \le \frac{1}{n}\Exp[Z_{h}^2\I\{\bw \in \cD_{h}\}] + \frac{1}{n}\Exp[Z_{h}^2\I\{\bw \notin \cD_{i,h}\}] \le \epsl^2 + B^2\frac{1}{n}\sum_{h=1}^n\Pr[\bw \notin \cD_{i,h}\}] \le \epsl^2 + B^2\epsmu$.
\end{proof}

\begin{proof} Let $M = |\cT|$, and let $\cE$ denote the event that
\begin{align*}
\cE_1 = \left\{\forall (i,j) \in [M]^2,  ~|\Delta(\theta_i,\theta_j;\bx_{1:n},\bw_{1:n})| \le \dtwo(\theta_i,\theta_j;\bx_{1:n})\sqrt{2\frac{B\log(2M/\delta)}{n}} + \frac{\log(2M/\delta)}{3n}\right\}
\end{align*}
and let 
\begin{align*}
\cE_2 = \left\{\sup_{\theta} \Delta(\theta,\theta_{i_{\cT}(\theta)};\bx_{1:n},\bw_{1:n})) \le \epsl +  2B\epsmu + \frac{B\log(M/\delta)}{2n}\right\}
\end{align*}
Then, on $\cE_{1} \cap \cE_2$, then for all $\theta,\theta'$ simultaneously, $\theta_i = \theta_{i_{\cT}(\theta)}$ and $\theta_{j} = \theta_{i_{\cT}(\theta')}$ satisfy
\begin{align*}
|\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n}))| &\le  |\Delta(\theta,\theta_{i};\bx_{1:n},\bw_{1:n}))| + |\Delta(\theta',\theta_{j};\bx_{1:n},\bw_{1:n}))| \\
&\quad+  |\Delta(\theta_{i},\theta_j;\bx_{1:n},\bw_{1:n}))| \\
&\le  \left(2\epsl +  4B\epsmu + \left(\frac{\log(M/\delta)}{n}\right) + \dtwo(\theta_i,\theta_j;\bx_{1:n})\sqrt{\frac{B\log(2M/\delta)}{n}} +  \frac{B\log(2M/\delta)}{3n}\right)\\
&\le  2\epsl +  4B\epsmu  + \dtwo(\theta_i,\theta_j;\bx_{1:n})\sqrt{\frac{\log(2M/\delta)}{n}} +  \frac{4B\log(2M/\delta)}{3n}\\
&\le  2\epsl +  4B\epsmu + \frac{\dtwo(\theta_i,\theta_j;\bx_{1:n})^2}{2\alpha B} +   \frac{(4+3\alpha)B\log(2M/\delta)}{3n}
\end{align*}
By the triangle inequality, 
\begin{align*}
\dtwo(\theta_i,\theta_j;\bx_{1:n}) &\le \dtwo(\theta,\theta';\bx_{1:n}) + \dtwo(\theta_i,\theta;\bx_{1:n}) + \dtwo(\theta_j,\theta';\bx_{1:n})\\
&\le \dtwo(\theta,\theta';\bx_{1:n}) + 2\sqrt{\epsl^2 + B^2\epsmu}\\
\end{align*}
Thus,
\begin{align*}
\dtwo(\theta_i,\theta_j;\bx_{1:n})^2 \le 2\dtwo(\theta,\theta';\bx_{1:n})^2 + 8\epsl^2 + 8B^2\epsmu^2
\end{align*}
Hence, 
\begin{align*}
|\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n}))| \le 2\epsl(1+\frac{2\epsl}{\alpha B}) +  4B\epsmu(1+\alpha^{-1}) + \frac{\dtwo(\theta_i,\theta_j;\bx_{1:n})^2}{2\alpha B} +   \frac{(4+3\alpha)B\log(2M/\delta)}{3n}
\end{align*}
Lastly, by taking $\epsl \le B$ and taking an $\inf$ over $\alpha$ we obtain on $\cE_1\cap\cE_2$ that
\begin{align*}
|\Delta(\theta,\theta';\bx_{1:n},\bw_{1:n}))| \le \inf_{\alpha > 0 } 4(1+\alpha^{-1})(\epsl + B\epsmu) + \frac{\dtwo(\theta_i,\theta_j;\bx_{1:n})^2}{2\alpha B} +   \frac{(4+3\alpha)B\log(2M/\delta)}{3n}
\end{align*}
\end{proof}
